Rethinking RGB Color Representation for Image Restoration Models

Image restoration models are typically trained with a pixel-wise distance loss defined over the RGB color representation space, which is well known to be a source of blurry and unrealistic textures in the restored images. The reason, we believe, is that the three-channel RGB space is insufficient for supervising the restoration models. To this end, we augment the representation to hold structural information of local neighborhoods at each pixel while keeping the color information and pixel-grainedness unharmed. The result is a new representation space, dubbed augmented RGB ($a$RGB) space. Substituting the underlying representation space for the per-pixel losses facilitates the training of image restoration models, thereby improving the performance without affecting the evaluation phase. Notably, when combined with auxiliary objectives such as adversarial or perceptual losses, our $a$RGB space consistently improves overall metrics by reconstructing both color and local structures, overcoming the conventional perception-distortion trade-off.

==> figures/result_deblur/main.tex <==
\begin{figure*}[b]
\newcommand{\figwidth}{0.165\linewidth}
\newcommand{\patchsize}{192_256}
\newcommand{\varA}{LQ}%
\newcommand{\varB}{Lchar}%
\newcommand{\varC}{LcharaRGB}%
\newcommand{\varD}{Lchar+TLC}%
\newcommand{\varE}{LcharaRGB+TLC}%
\newcommand{\varF}{GT}%
\centering
\vspace*{-1.6em}
\newcommand{\seed}{HIDE_34fromGOPR1089.MP4_255_575}%
    \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varA.png}}
    \hfill
    \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varB.png}}
    \hfill
    \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varC.png}}
    \hfill
    \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varD.png}}
    \hfill
    \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varE.png}}
    \hfill
    \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varF.png}}
    \\[-0.14em]
    \addtocounter{subfigure}{-6}
    \subfloat[Blurry\\ \hspace*{1.3em}\resizebox{3.5em}{!}{21.1887 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varA_diffmap.pdf}}
    \hfill
    \subfloat[$L_{\text{Char}}$\\ \hspace*{1.3em}\resizebox{3.5em}{!}{18.9074 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varB_diffmap.pdf}}
    \hfill
    \subfloat[{\color{BrickRed}$L_{\text{Char}, \text{$a$RGB}}$}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{\textbf{19.2360} $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varC_diffmap.pdf}}
    \hfill
    \subfloat[$L_{\text{Char}}\,$,TLC\\ \hspace*{1.3em}\resizebox{3.5em}{!}{19.3418 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varD_diffmap.pdf}}
    \hfill
    \subfloat[\resizebox{6em}{!}{{\color{BrickRed}$L_{\text{Char}, \text{$a$RGB}}\,$},TLC}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{\textbf{23.3990} $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varE_diffmap.pdf}}
    \hfill
    \subfloat[Clean GT\\ \hspace*{1.4em}\resizebox{3.5em}{!}{PSNR ($\mathrm{dB}$)}]{\vspace*{-1.02mm}\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varF_diffmap.pdf}}
% \newcommand{\seed}{HIDE_8fromGOPR1040.MP4_240_184}%
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varA.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varB.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varC.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varD.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varE.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varF.png}}
%     \\[-0.14em]
%     \addtocounter{subfigure}{-6}
%     \subfloat[Blurry\\ \hspace*{1.3em}\resizebox{3.5em}{!}{27.2154 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varA_diffmap.pdf}}
%     \hfill
%     \subfloat[$L_{\text{Char}}$\\ \hspace*{1.3em}\resizebox{3.5em}{!}{27.0476 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varB_diffmap.pdf}}
%     \hfill
%     \subfloat[{\color{BrickRed}$L_{\text{Char}, \text{$a$RGB}}$}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{\textbf{27.5802} $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varC_diffmap.pdf}}
%     \hfill
%     \subfloat[$L_{\text{Char}}\,$,TLC\\ \hspace*{1.3em}\resizebox{3.5em}{!}{27.2900 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varD_diffmap.pdf}}
%     \hfill
%     \subfloat[\resizebox{6em}{!}{{\color{BrickRed}$L_{\text{Char}, \text{$a$RGB}}\,$},TLC}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{\textbf{31.4381} $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varE_diffmap.pdf}}
%     \hfill
%     \subfloat[Clean GT\\ \hspace*{1.4em}\resizebox{3.5em}{!}{PSNR ($\mathrm{dB}$)}]{\vspace*{-1.02mm}\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varF_diffmap.pdf}}
% \newcommand{\seed}{GoPro_GOPR0410_11_00-000159_86_940}%
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varA.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varB.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varC.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varD.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varE.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varF.png}}
%     \\[-0.14em]
%     \addtocounter{subfigure}{-6}
%     \subfloat[Blurry\\ \hspace*{1.3em}\resizebox{3.5em}{!}{30.3011 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varA_diffmap.pdf}}
%     \hfill
%     \subfloat[$L_{\text{Char}}$\\ \hspace*{1.3em}\resizebox{3.5em}{!}{31.1395 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varB_diffmap.pdf}}
%     \hfill
%     \subfloat[{\color{BrickRed}$L_{\text{Char}, \text{$a$RGB}}$}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{\textbf{32.0593} $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varC_diffmap.pdf}}
%     \hfill
%     \subfloat[$L_{\text{Char}}\,$,TLC\\ \hspace*{1.3em}\resizebox{3.5em}{!}{32.5316 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varD_diffmap.pdf}}
%     \hfill
%     \subfloat[\resizebox{6em}{!}{{\color{BrickRed}$L_{\text{Char}, \text{$a$RGB}}\,$},TLC}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{\textbf{36.9283} $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varE_diffmap.pdf}}
%     \hfill
%     \subfloat[Clean GT\\ \hspace*{1.4em}\resizebox{3.5em}{!}{PSNR ($\mathrm{dB}$)}]{\vspace*{-1.02mm}\includegraphics[width=\figwidth]{figures/result_deblur/\seed_\patchsize_\varF_diffmap.pdf}}
% \\[-0.7em]
\\[-1em]
\caption{\small
    \textbf{Qualitative comparison of motion blur deblurring models trained with different loss functions.}
    %
    Each column corresponds to each row in Table~\ref{tab:result_deblur}.
    %
    % The network name and the common auxiliary loss $L_{\text{Edge}}$ are omitted from the captions.
    %
    The bottom row is the maximum absolute RGB difference.
}
\label{fig:result_deblur}
\end{figure*}

==> figures/result_denoise/main.tex <==
\begin{figure*}
\newcommand{\figwidth}{0.1418\linewidth}
\newcommand{\varA}{LQ}%
\newcommand{\varB}{N32}%
\newcommand{\varC}{N32+LPaRGB}%
\newcommand{\varD}{N32+L1aRGB}%
\newcommand{\varE}{N64}%
\newcommand{\varF}{N64+L1aRGB}%
\newcommand{\varG}{GT}%
\centering
\renewcommand{\seed}{0564}%
    \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varA.png}}
    \hfill
    \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varB.png}}
    \hfill
    \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varC.png}}
    \hfill
    \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varD.png}}
    \hfill
    \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varE.png}}
    \hfill
    \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varF.png}}
    \hfill
    \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varG.png}}
    \\[-0.05em]
    \addtocounter{subfigure}{-7}
    \subfloat[Noisy\\ \hspace*{1.3em}\resizebox{3.5em}{!}{17.1647 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varA_diffmap.pdf}}
    \hfill
    \subfloat[N32 $L_{\text{PSNR}}$\\ \hspace*{1.3em}\resizebox{3.5em}{!}{36.0312 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varB_diffmap.pdf}}
    \hfill
    \subfloat[{\scriptsize N32 {\color{BrickRed}$L_{\text{PSNR}, \text{$a$RGB}}$}}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{\textbf{36.3540} $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varC_diffmap.pdf}}
    \hfill
    \subfloat[\resizebox{4.9em}{!}{N32 {\color{BrickRed}$L_{1, \text{$a$RGB}}$}}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{\textbf{36.3747} $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varD_diffmap.pdf}}
    \hfill
    \subfloat[N64 $L_{\text{PSNR}}$\\ \hspace*{1.3em}\resizebox{3.5em}{!}{35.5460 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varE_diffmap.pdf}}
    \hfill
    \subfloat[\resizebox{4.9em}{!}{N64 {\color{BrickRed}$L_{1, \text{$a$RGB}}$}}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{\textbf{36.4639} $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varF_diffmap.pdf}}
    \hfill
    \subfloat[Clean GT\\ \hspace*{1.4em}\resizebox{3.5em}{!}{PSNR ($\mathrm{dB}$)}]{\vspace*{-0.72mm}\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varG_diffmap.pdf}}
% \newcommand{\seed}{1178}%
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varA.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varB.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varC.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varD.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varE.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varF.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varG.png}}
%     \\[-0.05em]
%     \addtocounter{subfigure}{-7}
%     \subfloat[Noisy\\ \hspace*{1.3em}\resizebox{3.5em}{!}{25.3056 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varA_diffmap.pdf}}
%     \hfill
%     \subfloat[N32 $L_{\text{PSNR}}$\\ \hspace*{1.3em}\resizebox{3.5em}{!}{39.1888 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varB_diffmap.pdf}}
%     \hfill
%     \subfloat[{\scriptsize N32 $L_{\text{PSNR}, \text{$a$RGB}}$}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{39.2866 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varC_diffmap.pdf}}
%     \hfill
%     \subfloat[\resizebox{4.9em}{!}{N32 $L_{1, \text{$a$RGB}}$}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{39.3632 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varD_diffmap.pdf}}
%     \hfill
%     \subfloat[N64 $L_{\text{PSNR}}$\\ \hspace*{1.3em}\resizebox{3.5em}{!}{39.3711 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varE_diffmap.pdf}}
%     \hfill
%     \subfloat[\resizebox{4.9em}{!}{N64 $L_{1, \text{$a$RGB}}$}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{40.1926 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varF_diffmap.pdf}}
%     \hfill
%     \subfloat[Clean GT]{\vspace*{-0.72mm}\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varG_diffmap.pdf}}
%     \\[-.7em]
% \newcommand{\seed}{0379}%
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varA.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varB.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varC.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varD.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varE.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varF.png}}
%     \hfill
%     \subfloat{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varG.png}}
%     \\[-0.05em]
%     \addtocounter{subfigure}{-7}
%     \subfloat[Noisy\\ \hspace*{1.3em}\resizebox{3.5em}{!}{29.4107 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varA_diffmap.pdf}}
%     \hfill
%     \subfloat[N32 $L_{\text{PSNR}}$\\ \hspace*{1.3em}\resizebox{3.5em}{!}{47.1689 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varB_diffmap.pdf}}
%     \hfill
%     \subfloat[{\scriptsize N32 {\color{BrickRed}$L_{\text{PSNR}, \text{$a$RGB}}$}}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{\textbf{47.5380} $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varC_diffmap.pdf}}
%     \hfill
%     \subfloat[\resizebox{4.9em}{!}{N32 {\color{BrickRed}$L_{1, \text{$a$RGB}}$}}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{\textbf{47.4457} $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varD_diffmap.pdf}}
%     \hfill
%     \subfloat[N64 $L_{\text{PSNR}}$\\ \hspace*{1.3em}\resizebox{3.5em}{!}{46.9483 $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varE_diffmap.pdf}}
%     \hfill
%     \subfloat[\resizebox{4.9em}{!}{N64 {\color{BrickRed}$L_{1, \text{$a$RGB}}$}}\\ \hspace*{1.3em}\resizebox{3.5em}{!}{\textbf{47.8430} $\mathrm{dB}$}]{\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varF_diffmap.pdf}}
%     \hfill
%     \subfloat[Clean GT\\ \hspace*{1.4em}\resizebox{3.5em}{!}{PSNR ($\mathrm{dB}$)}]{\vspace*{-0.72mm}\includegraphics[width=\figwidth]{figures/result_denoise/\seed_\varG_diffmap.pdf}}
    % \\[-.7em]
\\[-1em]
\caption{\small
    \textbf{Qualitative comparison of real image denoising models trained with different loss functions.}
    %
    Each column corresponds to each row in Table~\ref{tab:result_denoise}.
    %
    N32 corresponds to NAFNet-width32 and N64 corresponds to NAFNet-width64.
    %
    The bottom row shows the maximum absolute difference in color with a range of $[0, 1]\,$.
}
\label{fig:result_denoise}
\vspace*{-1.6em}
\end{figure*}

==> sections/figures/discussion_a.tex <==
\begin{figure}[t]
\centering
{%
\begin{minipage}{1.0\linewidth}    
    \subfloat[$\xx_{1}$]{\includegraphics[width=0.24\linewidth]{figures/discussion/src_rgb_v2.png}}
    \hspace{0.1mm}
    \subfloat[$\xx_{2}$]{\includegraphics[width=0.24\linewidth]{figures/discussion/src_extra_v2.png}}
    \hspace{0.1mm}
    \subfloat[\scriptsize{$f^{-1} (\xxi_{\text{mix}})$}]{\includegraphics[width=0.24\linewidth]{figures/discussion/opt_v2.png}}
    \hspace{0.1mm}
    \subfloat[\scriptsize{$\nabla^{2} f^{-1} (\xxi_{\text{mix}})$}]{\includegraphics[width=0.24\linewidth]{figures/discussion/opt_laplace_v2.png}}
\end{minipage}%
}
\vspace{-3mm}
\caption{
    \textbf{Inverting orthogonal mixture of two $a$RGB embeddings.}
}
\label{fig:discussion_a}
\vspace{-3mm}
\end{figure}

==> sections/figures/discussion_b.tex <==
\begin{figure}[t]
\centering
\hfill
\includegraphics[width=0.5\linewidth]{figures/discussion/segm_v2.pdf}
\hfill
\includegraphics[width=0.4\linewidth]{figures/discussion/tsne}
\\
\vspace{-3mm}
\caption{\textbf{(Left)~Expert Selection map of the MoE router~$f_{\text{r}}\,$. (Right)~t-SNE plot of the $a$RGB embedding $\xxi$ of pixels in the left image.}
    This provides compelling evidence that the features learned by our $a$RGB encoder $f$ are tailored to specific input structures, and even the embedding vectors within a single patch exhibit intricate clustering, thus supporting the rationale behind employing the Mixture of Experts~(MoE) architecture.
}
\label{fig:discussion_b}
\vspace{-3mm}
\end{figure}

==> sections/figures/discussion_c.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/discussion/dataset_metric_conversion.pdf}
\\
\vspace{-3mm}
\caption{\small
    \textbf{Change of $L_{2}$ metrics in the $a$RGB space relative to the $L_{2}$ metrics in the RGB space.}
    This shows how the distance metric changes in the $a$RGB space relative to the distance in the RGB space.
    Mean distances and their standard deviations are measured by MSE losses between an image and the same image with 100 AWGNs with the same standard deviation.
    Note that the $a$RGB space slightly exaggerates the distance more outside natural image domain, \eg, Gaussian noise, and the metric's variance is negligibly small.
}
\vspace{-3mm}
\label{fig:discussion_d}
\end{figure}

==> sections/figures/integration.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{example-image-a}
\vspace{-3mm}
\caption{
\small
\textbf{The overall pipeline of integrating our $a$RGB into existing restoration frameworks.}
From the pre-trained autoencoder, we employ the encoder~$f$ to transform RGB to the $a$RGB space.
Subsequently, we apply the pixel-wise loss between the restored and the ground truth images in the lifted $a$RGB space.
Note that the parameters of the encoder remain frozen during the training of the restoration model.
}
\label{fig:model_integration}
\vspace{-3mm}
\end{figure}

==> sections/tables/gan_deblur.tex <==
\begin{table}[t]
\begin{minipage}{.98\linewidth}
    \caption{\small
    \textbf{Results on real image denoising.}
    }
    \label{tab:result_denoise}
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{llcc}
        \toprule
        & & \multicolumn{2}{c}{{SIDD}} \\
        \cmidrule(lr){3-4} 
        Model & Objective & PSNR$\uparrow$ & SSIM$\uparrow$ \\
        \midrule
        NAFNet-width32 & $L_{\text{PSNR}}$ & 39.9672 & 0.9599 \\
        NAFNet-width32 & {\color{BrickRed} $L_{\text{PSNR}, \text{$a$RGB}}$ } & \textbf{39.9864} & \textbf{0.9601} \\
        NAFNet-width32 & {\color{BrickRed} $L_{1, \text{$a$RGB}}$} & \textbf{40.0106} & \textbf{0.9602} \\
        \cdashlinelr{1-4}
        NAFNet-width64 & $L_{\text{PSNR}}$ & 40.3045 & 0.9614 \\
        NAFNet-width64 & {\color{BrickRed} $L_{1, \text{$a$RGB}}$} & \textbf{40.3364} & \textbf{0.9620} \\
        \bottomrule
    \end{tabular}%
    }%
\end{minipage}
\vspace{-.1em}
\end{table}

